Quality Controlled Paraphrase Generation

Paraphrase generation has been widely used in various downstream tasks. Most tasks benefit mainly from high quality paraphrases, namely those that are semantically similar to, yet linguistically diverse from, the original sentence. Generating high-quality paraphrases is challenging as it becomes increasingly hard to preserve meaning as linguistic diversity increases. Recent works achieve nice results by controlling specific aspects of the paraphrase, such as its syntactic tree. However, they do not allow to directly control the quality of the generated paraphrase, and suffer from low flexibility and scalability. Here we propose $QCPG$, a quality-guided controlled paraphrase generation model, that allows directly controlling the quality dimensions. Furthermore, we suggest a method that given a sentence, identifies points in the quality control space that are expected to yield optimal generated paraphrases. We show that our method is able to generate paraphrases which maintain the original meaning while achieving higher diversity than the uncontrolled baseline. The models, the code, and the data can be found in https://github.com/IBM/quality-controlled-paraphrase-generation.

==> figures/ControlGlobal.tex <==
\begin{figure*}

\caption{Controlled paraphrase quality with the QP model neutralized. Average linguistic diversity (left column) and average semantic similarity (right column) of the paraphrases generated using the solution with the QP model neutralized vs. $o_syn$ and $o_lex$ for $o_{sem}=5$. Average is over the dev set. The number in each grid point is the difference from the uncontrolled baseline. Red/blue shades correspond to values above/below baseline.  \ranit{verify that the description is correct vs the final figure. also if we need more space we can consider referring to details in the caption of the other heatmap figure}}
\label{fig-heatmap-noref}
\end{figure*}
